Bubbles dynamics in microchannels: inertial and capillary migration forces

This work focuses on the dynamics of a train of unconfined bubbles flowing in microchan- nels. We investigate the transverse position of a train of bubbles, its velocity and the associated pressure drop when flowing in a microchannel depending on the internal forces due to viscosity, inertia and capillarity. Despite the small scales of the system, inertia, referred to as inertial migration force, play a crucial role in determining the transverse equilibrium position of the bubbles. Beside inertia and viscosity, other effects may also affect the transverse migration of bubbles such as the Marangoni surface stresses and the surface deformability. We look at the influence of surfactants in the limit of infinite Marangoni effect which yields rigid bubble interface. The resulting migration force may balance external body forces if present such as buoyancy, Dean or magnetic ones. This balance not only determines the transverse position of the bubbles but, consequently, the surrounding flow structure, which can be determinant for any mass/heat transfer process involved. Finally, we look at the influence of the bubble deformation on the equilibrium position and compare it to the inertial migration force at the centred position, explaining the stable or unstable character of this position accordingly. A systematic study of the influence of the parameters - such as the bubble size, uniform body force, Reynolds and capillary numbers - has been carried out using numerical simulations based on the Finite Element Method, solving the full steady Navier-Stokes equations and its asymptotic counterpart for the limits of small Reynolds and/or capillary numbers.

==> JFM Migration/Tables/matrizDPCircularLibre.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
0.93 \%&$i=0$&$i=2$&$i=4$&$i=6$\\%\hline
$j=0$&-0.06&0.52&-1.89&1.66\\%\hline
$j=2$&1.63&-9.67&53.58&-46.54\\%\hline
$j=4$&-14.96&125.05&-373.67&351.12\\%\hline
$j=6$&-10.97&-309.93&872.73&-672.23\\%\hline
$j=8$&31.08&278.73&-677.21&448.06\\%\hline
\end{tabular}


==> JFM Migration/Tables/matrizLCircularLibre.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
$\varphi=f_1$ & $i=1$ & $i=3$& $i=5$ &$i=7$\\%\hline
$j=1$&3.55&-7.42&-0.10&-0.51\\%\hline
$j=2$&-0.27&16.33&5.85&1.27\\%\hline
$j=3$&-4.67&7.65&-7.98&-38.37\\%\hline
$j=4$&0.45&-43.31&-14.05&100.91\\%\hline
$j=5$&-0.79&28.12&19.56&-68.44\\%\hline
\end{tabular}


%%% 0.21 \%


==> JFM Migration/Tables/matrizLCircularRigido.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
$\varphi=f_1$&$i=1$&$i=3$&$i=5$&$i=7$\\%\hline
$j=1$&13.28&-33.15&2.20&-0.63\\%\hline
$j=2$&-43.14&115.27&19.72&-28.76\\%\hline
$j=3$&48.60&-104.32&-137.39&122.41\\%\hline
$j=4$&-20.20&-36.05&255.14&-177.07\\%\hline
$j=5$&0.57&65.47&-150.87&89.05\\%\hline
\end{tabular}


%%0.15 \%


==> JFM Migration/Tables/matrizOmCircularRigido.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
$\varphi=\Omega_0/8 \varepsilon$ &$i=0$&$i=2$&$i=4$&$i=6$\\%\hline
$j=0$&1.00&-0.02&0.12&-0.20\\%\hline
$j=2$&-0.14&-0.42&-0.93&-0.98\\%\hline
$j=4$&-0.77&1.30&1.00&10.63\\%\hline
$j=6$&0.94&-2.40&6.04&-31.08\\%\hline
$j=8$&-0.62&2.43&-10.59&29.65\\%\hline
\end{tabular}

%%%0.14 \%


==> JFM Migration/Tables/matrizV_VPCircularLibre.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
$ \varphi=V_0/V_P$&$i=0$&$i=2$&$i=4$&$i=6$\\%\hline
$j=0$&1.00&-0.01&0.04&-0.07\\%\hline
$j=2$&0.02&-0.17&0.26&-1.56\\%\hline
$j=4$&-0.32&-0.02&-2.70&7.93\\%\hline
$j=6$&-1.05&0.32&6.87&-15.38\\%\hline
$j=8$&0.94&0.07&-5.67&11.28\\%\hline
\end{tabular}
%%% 0.08 \%

==> JFM Migration/Tables/matrizV_VPCircularRigido.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
$ \varphi=V_0/V_P$  &$i=0$&$i=2$&$i=4$&$i=6$\\%\hline
$j=0$&1.00&-0.02&0.10&-0.20\\%\hline
$j=2$&-0.67&-0.63&-1.07&-0.47\\%\hline
$j=4$&0.05&2.42&4.19&5.87\\%\hline
$j=6$&0.31&-3.47&-7.35&-14.90\\%\hline
$i=8$&-0.22&1.95&4.88&12.49\\%\hline
\end{tabular}
%%% 0.18 \%

==> JFM Migration/Tables/matrizbeta100CircularLibre.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
$\varphi=100 \beta_0$&$i=0$&$i=2$&$i=4$&$i=6$\\%\hline
$j=0$&-0.03&0.31&-1.11&0.98\\%\hline
$j=2$&0.95&-5.67&31.40&-27.27\\%\hline
$j=4$&-8.76&73.27&-218.95&205.73\\%\hline
$j=6$&-6.43&-181.60&511.37&-393.88\\%\hline
$j=8$&18.21&163.32&-396.80&262.54\\%\hline
\end{tabular}
%% 0.93 \%

==> JFM Migration/Tables/matrizbeta100CircularRigido.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
$\varphi=100 \beta_0$  &$i=0$&$i=2$&$i=4$&$i=6$\\%\hline
$j=0$&-0.01&0.14&-0.68&0.45\\%\hline
$j=2$&0.23&3.65&16.84&-9.38\\%\hline
$j=4$&3.44&60.06&-95.98&116.73\\%\hline
$j=6$&18.31&-130.40&171.85&-146.87\\%\hline
$j=8$&12.72&105.94&-100.60&50.42\\%\hline
\end{tabular}
%%%0.30 \%

==> JFM Migration/Tables/matrizfdatos_Ca0.tex <==
\begin{tabular}{|c|c|c|c|c|}
%\hline
$\varphi=f_1$& $i=1$&$i=3$&$i=5$&$i=7$\\%\hline
$j=1$&-104.96&-238.40&1115.32&-1865.91\\%\hline
$j=3$&9.20&-608.76&-2701.91&1727.04\\%\hline
$j=5$&-1287.13&-26449.45&162691.63&-246331.61\\%\hline
$j=7$&3666.66&94964.56&-547128.86&839403.47\\%\hline
$j=9$&-4931.48&-140975.28&775574.28&-1203791.84\\%\hline
\end{tabular}

%%%%1.18 \%

==> Tables/matrizDPCircularLibre.tex <==
\begin{tabular}{|c|r|r|r|r|}
%\hline
0.93 \%&$i=0$&$i=2$&$i=4$&$i=6$\\%\hline
$j=0$&-0.06&0.52&-1.89&1.66\\%\hline
$j=2$&1.63&-9.67&53.58&-46.54\\%\hline
$j=4$&-14.96&125.05&-373.67&351.12\\%\hline
$j=6$&-10.97&-309.93&872.73&-672.23\\%\hline
$j=8$&31.08&278.73&-677.21&448.06\\%\hline
\end{tabular}

